SuperConga: an open-source framework for mesoscopic superconductivity

We present SuperConga, an open-source framework for simulating equilibrium properties of unconventional and ballistic singlet superconductors, confined to two-dimensional (2D) mesoscopic grains in a perpendicular external magnetic field, at arbitrary low temperature. It aims at being both fast and easy to use, enabling research without access to a computer cluster, and visualization in real-time with OpenGL. The core is written in C++ and CUDA, exploiting the embarrassingly parallel nature of the quasiclassical theory of superconductivity by utilizing the parallel computational power of modern GPUs. The framework self-consistently computes both the superconducting order-parameter and the induced vector potential, and finds the current density, free energy, induced flux density, local density of states, as well as the magnetic moment. A user-friendly Python frontend is provided, enabling simulation parameters to be defined via intuitive configuration files, or via the command-line interface, without requiring a deep understanding of implementation details. For example, complicated geometries can be created with relative ease. The framework ships with simple tools for analyzing and visualizing the results, including an interactive plotter for spectroscopy. An overview of the theory is presented, as well as examples showcasing the framework's capabilities and ease of use. The framework is free to download from https://gitlab.com/superconga/superconga, which also links to the extensive user manual, containing even more examples, tutorials and guides.

==> app_output_format.tex <==
\section{Data output format}
\label{app:data_output}

The results produced by the SuperConga framework are saved as human-readable data files with standard file formats. Scalar data and settings are saved in \texttt{json}-files. Quantities that depend on coordinates (or other variables) are saved as \texttt{csv}-files (Comma-Separted Values), where data is stored in comma-separated columns with a header describing the contents of each column. For example, the total current density is saved in the file \texttt{current\_density.csv}, with columns for discrete $x$- and $y$-coordinates (called \texttt{x\_idx} and \texttt{y\_idx}), and columns for the $x$- and $y$-components of the current (called \texttt{j\_x} and \texttt{j\_y}). Having parsed this data, the discrete coordinates can be transformed to physical coordinates in units of coherence lengths by multiplying \texttt{x\_idx} and \texttt{y\_idx} with the discretization size. The latter is saved under the field ``\texttt{points\_per\_coherence\_length}'' in the file \texttt{config.json}. By using these standard file-formats, it is straightforward for the user to post-process and visualize the results with their favorite tools. Still, to facilitate even further for the user, SuperConga comes with some existing post-processing tools (written in C++/CUDA and Python) for visualizing and analysing the data.
